Leveraging Image Augmentation for Object Manipulation: Towards Interpretable Controllability in Object-Centric Learning

The binding problem in artificial neural networks is actively explored with the goal of achieving human-level recognition skills through the comprehension of the world in terms of symbol-like entities. Especially in the field of computer vision, object-centric learning (OCL) is extensively researched to better understand complex scenes by acquiring object representations or slots. While recent studies in OCL have made strides with complex images or videos, the interpretability and interactivity over object representation remain largely uncharted, still holding promise in the field of OCL. In this paper, we introduce a novel method, Slot Attention with Image Augmentation (SlotAug), to explore the possibility of learning interpretable controllability over slots in a self-supervised manner by utilizing an image augmentation strategy. We also devise the concept of sustainability in controllable slots by introducing iterative and reversible controls over slots with two proposed submethods: Auxiliary Identity Manipulation and Slot Consistency Loss. Extensive empirical studies and theoretical validation confirm the effectiveness of our approach, offering a novel capability for interpretable and sustainable control of object representations.

==> Main/Partials/alg_slota.tex <==
% slot attention - spatial binding
\begin{algorithm}[H]
	\caption{
 Spatial binding in slot attention algorithm in pseudo-code format. 
 The input image is encoded into a set of $N$ vectors of dimension $D_{input}$ which is mapped to a set of $K$ vectors with dimension  $D_{slot}$. 
 Slots are initialized from a Gaussian distribution with learned parameters $\mu, \sigma \in \mathbb{R}^{D_{slot}}$. 
 The number of iterations is set to $T = 3$.} 
 
	\begin{algorithmic}[1]
        \Function{\text{SpatialBinding}}{$\texttt{img} \in \mathbb{R}^{H \times W \times 3}$}
            \State $\texttt{inputs} = \texttt{Encoder(img)}$
            % \State $\texttt{inputs} \in \mathbb{R}^{N \times D_{\text{enc}}}= \texttt{Encoder(img)}$
            \State $\texttt{inputs} = \texttt{LayerNorm(inputs)}$
            \For{$t = 0 \ldots T$}
                \State $\texttt{slots\_prev} = \texttt{slots}$
                \State $\texttt{slots} = \texttt{LayerNorm(slots)}$
                \State $\texttt{attn} = \texttt{Softmax}(\frac{1}{\sqrt{D_{slot}}}k(\texttt{inputs})\cdot q(\texttt{slots})^T, \texttt{axis=`slots'})$
                \State $\texttt{updates} = \texttt{WeightedMean(weights=attn+}\epsilon \texttt{, values=} v\texttt{(inputs))}$
                \State $\texttt{slots} = \texttt{GRU(state=slots\_prev, inputs=updates)}$
                \State $\texttt{slots} = \texttt{slots} + \texttt{MLP(LayerNorm(slots))}$
            \EndFor
            \State \textbf{return} \texttt{slots}
        \EndFunction
    \end{algorithmic} 
\label{alg:slota}
\end{algorithm} 
% https://www.overleaf.com/project/644229399c32fba85749b80a

==> Main/Partials/fig_exp_manip.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Main/Assets/exp_manip_v0.pdf}
    \vspace{-1em}
    \caption{
    \textbf{Examples of object-level manipulation.}
    The text on each image states the instruction used for manipulation.
    The top two rows show the manipulation cases for CLEVR6 dataset, \textcolor{red}{and the last row shows the case for Tetrominoes.}}
    \label{fig:exp_manip}
\end{figure}

==> Main/Partials/table.tex <==

\begin{table*}[t]

% % ============ od and manip (including MSE) ============
% \begin{minipage}[t]{0.55\linewidth}
% \setlength{\tabcolsep}{6pt}
% \begin{center}
% \caption{
% Results on object discovery and image reconstruction tasks. mIoU and ARI are reported in \% (mean $\pm$ std for 3 trials).
% }
% \label{tab:od_and_recon}
% \begin{tabular}{lccc}
% \toprule
%  & mIoU ($\uparrow$) & ARI ($\uparrow$) & \multicolumn{1}{c}{MSE} ($\downarrow$) \\ \hline
%  & \multicolumn{3}{c}{Previous methods} \\ \hline
% SA \citep{locatello2020object} & 47.3 $\pm$ 23.2 & 63.1 $\pm$ 54.5 & \textbf{2.69e-4} \\
% +ARK \citep{kim2023shepherding} & \textbf{68.8 $\pm$ \phantom{0}0.4}  & \textbf{95.4 $\pm$ \phantom{0}0.5} & 2.81e-4 \\ \hline
% & \multicolumn{3}{c}{Ours} \\ \hline
% v1 & \textbf{68.9 $\pm$ \phantom{0}0.1} & \textbf{95.7 $\pm$ \phantom{0}0.2} & 3.25e-4 \\
% v2 & 68.5 $\pm$ \phantom{0}0.1 & 95.3 $\pm$ \phantom{0}0.1 & 3.41e-4 \\
% v3 & 68.5 $\pm$ \phantom{0}0.1 & \textbf{95.2 $\pm$ \phantom{0}0.7} & 3.29e-4 \\
% \bottomrule

% \end{tabular}
% \end{center}
% \end{minipage} 

% \hfill


% ============ od and manip ============
\begin{minipage}[t]{0.62\linewidth}
\setlength{\tabcolsep}{6pt}\begin{center} 
\caption{
\textbf{Results on object discovery.} Two metrics, mean Intersection over Union (mIoU) and Adjusted Rand Index (ARI) are reported in \% (mean $\pm$ std for 3 trials) \textcolor{blue}{on CLEVR6}. 
}
\label{tab:od_and_recon}
\begin{tabular}{lcc}
\toprule
 & mIoU ($\uparrow$) & ARI ($\uparrow$) \\ \hline
 \multicolumn{1}{c}{Previous methods} & &  \\ \hline
SA \citep{locatello2020object} & 47.3 $\pm$ 23.2 & 63.1 $\pm$ 54.5 \\
+ARK \citep{kim2023shepherding} & \textbf{68.8 $\pm$ \phantom{0}0.4}  & \textbf{95.4 $\pm$ \phantom{0}0.5} \\ \hline
\multicolumn{1}{c}{Ours (SlotAug)} & & \\ \hline
Base model (v1) & \textbf{68.9 $\pm$ \phantom{0}0.1} & \textbf{95.7 $\pm$ \phantom{0}0.2} \\
+ AIM (v2) & 68.5 $\pm$ \phantom{0}0.1 & 95.3 $\pm$ \phantom{0}0.1 \\
+ AIM + SCLoss (v3) & 68.5 $\pm$ \phantom{0}0.1 & \textbf{95.2 $\pm$ \phantom{0}0.7} \\
\bottomrule

\end{tabular}
\end{center}
\end{minipage} 
\hfill
% ============ durabilitiy ============
\begin{minipage}[t]{0.33\linewidth}
\setlength{\tabcolsep}{6pt}

\begin{center}
\caption{
\textbf{Results on durability test} with MSE on CLEVR6.
% S- and O- represents slots and objects.
}
\label{tab:durability}
\begin{tabular}{lcc}
\toprule
 % & S-RMSE ($\downarrow$) & O-Pos. ($\downarrow$) \\ \hline
 & Slot ($\downarrow$) & Obj. Pos. ($\downarrow$) \\ \hline
 & \multicolumn{2}{c}{Single step (x8)} \\ \hline
v1 & 50.8 & 0.14 \\
v2 & 39.7 & 0.15 \\
v3 & \textbf{0.25} & \textbf{0.01} \\ \hline
 & \multicolumn{2}{c}{Multiple steps (x4)} \\ \hline
v1 & 54.0 & 0.16 \\
v2 & 41.4 & 0.11 \\
v3 & \textbf{0.31} & \textbf{0.02} \\
\bottomrule
\end{tabular}
\end{center}
\end{minipage}

\end{table*}


==> Main/Sections/preliminaries.tex <==
\vspace{-0.5em}
\section{Preliminary: Slot Attention}
\vspace{-1em}
\input{Main/Partials/alg_slota}
\vspace{-0.7em}
Slot Attention \cite{locatello2020object} introduces the concept of \textit{slots}, a set of $K$ vectors of dimension $D_{slot}$, that serve as the object-centric representation.
The slots are initialized by a Gaussian distribution with learnable mean $\mu$ and sigma $\sigma$, and are updated over $T$ iterations by the slot attention module.
The final slots are then decoded to reconstruct the target image.
% To provide comprehensive understanding of our method, we describe the \textsc{SpatialBinding} function in \Cref{alg:slota}. The SpatialBinding function represents the mechanisim of the slot attention.
To provide a comprehensive understanding of our method, we describe the mechanism of the slot attention, \textsc{SpatialBinding}, in Alg. \ref{alg:slota}.
% Given an input image \texttt{img} $\in \mathbb{R}^{H \times W \times 3}$, convolutional neural networks (CNNs) encoder generates a visual feature map \texttt{input} $\in \mathbb{R} ^ {N \times D_{enc}}$, where $H$, $W$, $N$, and $D_{\text{enc}}$ are the height and width of the input image, the number of pixels in the input image ($= HW$), and the channel of the visual feature map. 
% The slot attention module takes \texttt{slots} and \texttt{inputs}, and projects them to dimension $D_{slot}$ through linear transformations $k$, $q$, and $v$.
% Dot-product attention is applied to generate an attention map, \texttt{attn}, with query-wise normalized coefficients, enabling slots to compete for the most relevant pixels of the visual feature map.
% The attention map coefficients weight the projected visual feature map to produce updated slots, \texttt{updates}.
% With the iterative mechanism of the slot attention module, the slots can gradually refine their representations. 
Each updated slot is then decoded individually into an RGBA image using a spatial broadcast decoder \cite{watters2019spatial} which is shared across slots. 
The decoded images are blended into a single image using alpha masks to reconstruct the input image.
% The training objective function is the mean squared error (MSE) between the original input image and the reconstructed image, following an unsupervised learning approach.
The training objective is the mean squared error (MSE) between the original input image and the reconstructed image, following an unsupervised learning approach.



==> Rebuttal/Partials/fig_complex.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Rebuttal/Assets/complex.pdf}
    % \vspace{-1em}
    \caption{
    \textbf{Results of the proposed method for the complex datasets.}
    asdf
    }
    \label{fig:complex}
\end{figure}


==> Rebuttal/Partials/fig_unmanip.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Rebuttal/Assets/unmanip.pdf}
    % \vspace{-1em}
    \caption{
    \textbf{Results of the image composition with manipulated slots.}
    asdf
    }
    \label{fig:complex}
\end{figure}


==> Rebuttal/Sections/figures.tex <==
\input{Rebuttal/Partials/fig_complex}

\input{Rebuttal/Partials/fig_unmanip}

==> match_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

